Comparing HAWC blazars light curves with different data reconstruction versions

We present a comparison of the flux normalization of HAWC sources using 17 months of data that was processed using two different versions of the official data reconstruction used for HAWC analyses. Pass4 (P4) has been used so far for most of the results published by HAWC. The most recent reconstruction version, Pass5 (P5) will be used in future analyses and comes with better pointing accuracy and improved gamma/hadron separation. The aim of this work is to do a comparison of the light curves obtained with both P4 and P5 and show that the results are consistent within statistical uncertainties

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

